'Tax-free' 3DMM Conditional Face Generation

3DMM conditioned face generation has gained traction due to its well-defined controllability; however, the trade-off is lower sample quality: Previous works such as DiscoFaceGAN and 3D-FM GAN show a significant FID gap compared to the unconditional StyleGAN, suggesting that there is a quality tax to pay for controllability. In this paper, we challenge the assumption that quality and controllability cannot coexist. To pinpoint the previous issues, we mathematically formalize the problem of 3DMM conditioned face generation. Then, we devise simple solutions to the problem under our proposed framework. This results in a new model that effectively removes the quality tax between 3DMM conditioned face GANs and the unconditional StyleGAN.

==> figures/fig_qualitative_disentanglement/fig_qualitative_disentanglement.tex <==

{   % Scope declared variables

\begin{figure}[t]
    \centering

    \includegraphics[width=1\linewidth]{./figures/fig_qualitative_disentanglement/68041_compare.pdf}
    \vspace{-0.5cm}
    \caption{Real face editing. After inversion, for which all methods show some error, our model shows competitive ability. In both inversion and individual attribute edits, our model generates images that are faithful to the 3DMM renderer outputs and the original image.
	}
    \label{fig:qualitative_synthetic}
    \vspace{-0.3cm}
\end{figure}

}

==> tables/table_ablation.tex <==
\begin{table}[t]
    \caption{FID and Disentanglement Score comparisons between all ablation experiments}
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tabular}{l|lllll}
        \hline
        Method & \multicolumn{1}{l|}{Quality} & \multicolumn{4}{l}{Disentanglement Score} \\ \hline
         & \multicolumn{1}{l|}{FID$\downarrow$} & id$\uparrow$ & exp$\uparrow$ & illum$\uparrow$ & angle$\uparrow$ \\ \hline
        Config-A & \textbf{8.73} & 1.07 & 3.19 & 49.5 & 1402 \\
        Config-B & 17.5 & \textbf{1.14} & \textbf{5.97} & \textbf{57.2} & \textbf{1964} \\
        Config-C & 10.9 & 0.694 & 2.71 & 29.2 & 1142 \\
        Config-D & 13.3 & 0.41 & 1.25 & 23.2 & 690 \\ \hline
        \end{tabular}
        }
    \label{tab:ablation}
    \vspace{-0.3cm}
\end{table}

==> tables/table_dci.tex <==
\begin{table}[t]
    \caption{DCI metric comparisons.}
        \centering
        % \begin{tabular}{ lr }
        %     \toprule
        %     Method & Full Sequence Accuracy\\
        %     \midrule
        %     Simple Mouth & 0.04\\
        %     DWT & 0.96 \\
        %     Ours & \textbf{1.00}\\
        %     \bottomrule
        % \end{tabular} \quad
        \resizebox{\linewidth}{!}{
        \begin{tabular}{ l|ccc }
            \toprule
            Method & Disentanglement$\uparrow$ & Completeness$\uparrow$ & Informativeness$\uparrow$ \\
            \midrule
            DiscoFaceGAN & 0.66 & 0.73 & 0.98 \\
            Ours & \textbf{0.83} & \textbf{0.78} & \textbf{0.99} \\
            \bottomrule
        \end{tabular}
        }
    \label{tab:dci}
    \vspace{-0.3cm}
\end{table}

==> tables/table_disentanglement_score.tex <==
\begin{table}[t]
    \caption{Disentanglement Score comparisons with DiscoFaceGAN across four 3DMM-controlled attributes.}
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tabular}{ l|cccc }
            \toprule
            Method & $DS_{\text{id}}\uparrow $ & $DS_{\text{exp}}\uparrow$ & $DS_{\text{illum}}\uparrow$ & $DS_{\text{angle}}\uparrow$ \\
            \midrule
            DiscoFaceGAN & 0.37 & 1.64 & 47.9 & 829 \\
            Ours & \textbf{1.02} & \textbf{3.22} & \textbf{48.7} & \textbf{1245} \\
            \bottomrule
        \end{tabular}
        }
    \label{tab:ds}
    \vspace{-0.3cm}
\end{table}

==> tables/table_quality.tex <==
\begin{table}[t]
    \caption{Our conditioning provides control and almost equivalent quality to unconditioned baseline StyleGAN2. Two baseline 3DMM conditioning approaches do not produce comparable quality in terms of FID. P\&R were introduced after StyleGAN1 and thus these numbers are missing from DiscoFaceGAN (built on StyleGAN1). }
    \vspace{0.1cm}
    \centering
    %\resizebox{\linewidth}{!}{
    \begin{tabular}{ l|ccc }
        \toprule
        Method & FID$\downarrow$ & Precision$\uparrow$ & Recall$\uparrow$ \\
        \midrule
        StyleGAN2 & 3.78 & 0.692 & 0.431 \\
        Ours & 4.51 & 0.574 & 0.485 \\
        DiscoFaceGAN & 12.9 & - & - \\
        3D-FM GAN & 12.2 & - & - \\
        \bottomrule
    \end{tabular}
    %}
    \label{tab:quality}
\end{table}

==> tex/02_relatedwork.tex <==
\section{Related Work}

Given the specificity of our contribution, we discuss a limited slice of works that explains 3DMM-conditioned GANs.

\vspace{-0.1cm}
\paragraph{Face generation using GANs and disentangling.}
In 2017, with the introduction of PGGAN~\cite{pggan}, the long-standing challenge of generating high resolution images had its first breakthrough, and Karras et al.'s StyleGAN family~\cite{sg1,sg2,sg3} has been the state-of-the-art in single domain image synthesis since then. A natural subsequent task is controlled generation of photorealistic images using StyleGAN. Despite numerous attempts ~\cite{interfacegan, Shen_2021_CVPR, stylespace, stylemorph}, achieving both image quality and controllability remains challenging due to the lack of tractable semantics in StyleGAN's latent spaces. 

% Generative Adversarial Networks (GANs) ~\cite{gan} are widely used to generate realistic images. A GAN trained on a large dataset of real human faces such as FFHQ~\cite{ffhq} is capable of generating almost indistinguishable pictures of human appearances from real photographs. In particular, StyleGAN is a highly influential model in the field that has inspired many new research directions and applications. One of the key innovations of StyleGAN is that the generator gradually increases the resolution of the images while injecting the image style, which helps to prevent the network from getting stuck in local minima and allows it to generate images with high fidelity. StyleNeRF is another generative model which uses a hybrid network architecture that combines the two models, where the NeRF model is used to create a 3D representation of the scene and then the StyleGAN model to add disentangled style and appearance to the rendered image.

% This sentence does not belong here
% As a major component in mainstream face recognition methods, image synthesis for human faces has long been a topic of interest in the scientific world ~\cite{lu2017faceimagesynthesis}. Controllable face synthesis is one of its sub task and is specified as such: given an input human face, a model needs to generate a photorealistic human face with some modified facial attribute(s) while preserving the others.

% Due to the high-quality face-generation capability of GANs and/or their inherent latent space, many studies rely on them for latent space editing. This empowers their networks to manipulate a person's expression, age, pose, etc. InterFaceGan by Shen \etal~\cite{shen2020interpreting} trained SVMs to find the hyperplane in StyleGAN latent space for each of the facial attributes and used vector arithmetic to achieve conditional attribute manipulation in Z space. Built upon InterFaceGan, Wang \etal ~\cite{wang2021HFGI} explored the Rate-Distortion tradeoffs between the image editability and reconstruction quality of StyleGAN's latent space and achieved high fidelity in both editing and reconstruction. On the other hand, GANspace by Härkönen \etal~\cite{ganspace} performed unsupervised learning, mainly PCA, on the latent space in StyleGAN as well as feature layers in BigGAN to find the directions of some editable features.

\vspace{-0.1cm}
\paragraph{3D prior for face modeling and synthesis.}
Numerous 3D methods for face generation exist. Among these, 3D Morphable Models (3DMMs)~\cite{paysan20093d, guo2018cnn} constitute a statistical approach that embeds human faces into a parameter space consisting of a set of principal components that represent factors including identity, expression, illumination, and pose. In contrast, Neural Radiance Fields (NeRFs)~\cite{nerf} generate photorealistic 3D scenes by leveraging a learned neural network to model the implicit 3D geometry and appearance of the target. While a number of 3D-aware models~\cite{stylenerf, pigan} have incorporated NeRFs to synthesize facial images with pose variations, this approach is very computationally expensive.

\vspace{-0.1cm}
\paragraph{3DMM-conditioned StyleGAN.}
The semantic interpretability of 3DMM offers the potential for controllable generation of faces. Proposed works combine 3DMM and StyleGAN to try to gain both semantic control and image quality. One type of such work~\cite{dfg,3fg, sun2022controllable} \textit{conditions} their model training on the 3DMM parameter space, but the added control constraints the output quality. In contrast, another type of work~\cite{stylerig} \textit{rigs} the StyleGAN latent space, producing higher quality results but restricting control.

\vspace{-0.1cm}
\paragraph{Disentangled representation learning (DRL).}
DRL~\cite{bengio2013representation} aims to represent and disentangle the constitutional factors lying in the data of interest. Many studies have sought to apply DRL to GAN for disentangled face synthesis. In particular, InfoGAN~\cite{infogan} and its variants ~\cite{infogan-cr, pg-infogan} attempt to maximize the mutual information between latent codes and generated samples to enforce disentangling. Peebles~\etal~\cite{peebles2020hessian} design a regularization term that encourages the Hessian of a model with respect to its input to be diagonal, thereby minimizing the interdependence of target factors.

% \subsection{3D Face Modeling and Synthesis}
% 3D Morphable Models (3DMM) reflect human faces with a set of principal components representing identity, expression, pose, texture, and illumination. There are many proposed research works that estimate 3DMM parameters from 2D images to gain 3D awareness, including methods that use 3DMM as a prior, which we call pre-hoc methods~\cite{uvgan, Gecer_2018, dfg}. In particular, DiscoFaceGAN~\cite{dfg} is trained with 3DMM coefficient vectors during the training stage, but these are not required for rendering the result. 
% cGOF++~\cite{cgof} also incorporates 3DMM priors but it is a conditional 3D generative model based on Neural Radiance Field (NeRF) which uses two auxiliary volumetric losses including 3D landmark loss and column warping loss.

% 3D Controllable Face Manipulation GAN (3D-FM GAN)~\cite{3fg} is another pre-hoc model which utilizes a face reconstruction network \textbf{FR} to estimate some 3DMM parameters $p$ of the input face (identity, expression, illumination, pose), then after manipulating some of the parameters, the new $p'$ is sent to a renderer \textbf{Rd} to generate the manipulated photo.


% StyleRig~\cite{stylerig} contains a Differentiable Face Reconstruction (DFR) network which maps a latent \paragraph{3DMM-Conditioned StyleGAN} code \textbf{w} to a set of semantic control parameters $p_w$ which can be used to concatenated with the output of the RigNet encoder to produce a vector \textbf{d} in the decoder. \textbf{d} is served as the discrepancy of the original latent vector \textbf{w} so that a new latent vector \textbf{\^{w}} can be obtained and used to generate faces with StyleGAN. We call such model post-hoc methods. A different RigNet was trained for different modes of control, including pose, expressions, and illumination. Portrait Image Embedding (PIE)~\cite{pie} which was built upon StyleGAN and StyleRig, on the other hand, is able to edit real images rather than only synthetic ones.

% \subsection{Controllable and Disentangled Face Models}

